Dual-Hybrid Attention Network for Specular Highlight Removal

Specular highlight removal plays a pivotal role in multimedia applications, as it enhances the quality and interpretability of images and videos, ultimately improving the performance of downstream tasks such as content-based retrieval, object recognition, and scene understanding. Despite significant advances in deep learning-based methods, current state-of-the-art approaches often rely on additional priors or supervision, limiting their practicality and generalization capability. In this paper, we propose the Dual-Hybrid Attention Network for Specular Highlight Removal (DHAN-SHR), an end-to-end network that introduces novel hybrid attention mechanisms to effectively capture and process information across different scales and domains without relying on additional priors or supervision. DHAN-SHR consists of two key components: the Adaptive Local Hybrid-Domain Dual Attention Transformer (L-HD-DAT) and the Adaptive Global Dual Attention Transformer (G-DAT). The L-HD-DAT captures local inter-channel and inter-pixel dependencies while incorporating spectral domain features, enabling the network to effectively model the complex interactions between specular highlights and the underlying surface properties. The G-DAT models global inter-channel relationships and long-distance pixel dependencies, allowing the network to propagate contextual information across the entire image and generate more coherent and consistent highlight-free results. To evaluate the performance of DHAN-SHR and facilitate future research in this area, we compile a large-scale benchmark dataset comprising a diverse range of images with varying levels of specular highlights. Through extensive experiments, we demonstrate that DHAN-SHR outperforms 18 state-of-the-art methods both quantitatively and qualitatively, setting a new standard for specular highlight removal in multimedia applications.

==> figtex/teaser.tex <==
\begin{teaserfigure}
  \begin{minipage}[b]{1.0\linewidth}
        \begin{minipage}[b]{0.19\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{example-image-a}}
            \centerline{(a)}\medskip
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.19\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{example-image-a}}
            \centerline{(b)}\medskip
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.19\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{example-image-a}}
            \centerline{(c)}\medskip
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.19\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{example-image-a}}
            \centerline{(d)}\medskip
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.19\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{example-image-a}}
            \centerline{(e)}\medskip
        \end{minipage}
    \end{minipage}
  \caption{Seattle Mariners at Spring Training, 2010.}
  \label{fig:teaser}
\end{teaserfigure}

==> tabletex/1_quan_horiztl.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{{\small The quantitative comparison results, positioning 11 traditional methods on the left and 7 learning-based approaches on the right. The highest-performing results are emphasized in bold, while the second-best are underscored.}}
\adjustbox{width=\textwidth}{%
\begin{tabular}{|cc|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Method}     &  \cite{1374865} &  \cite{yoon2006fast} &  \cite{shen2008chromaticity} &  \cite{shen2009simple} & \cite{yang2010real} & \cite{shen2013real} & \cite{akashi2015separation} & \cite{huo2015hdr} & \cite{fu2019specular} & \cite{yamamoto2019general} & \cite{saha2020combining} & \cite{guo2018single} & \cite{fu2021multi} & \cite{wu2021single} & \cite{hu2022mask} & \cite{wu2023joint} & \cite{fu2023towards} & \cite{hu2024highlight} & Ours \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{PSD}}  & PSNR$\uparrow$  & 5.44  & 16.09 & 19.56 & 21.33 & 4.74  & 11.51 & 17.48 & 20.16 & 15.24 & 18.37 & 15.98 & 13.25 & 22.78 & 23.58 & 22.12 & 23.93 & 23.30 & 20.79 & 25.20 \\ \cline{2-21} 
\multicolumn{1}{|c|}{}                      & SSIM$\uparrow$  & 0.218 & 0.498 & 0.666 & 0.753 & 0.250 & 0.324 & 0.565 & 0.767 & 0.688 & 0.541 & 0.455 & 0.571 & 0.811 & 0.838 & 0.815 & 0.863 & 0.826 & 0.845 & 0.882 \\ \cline{2-21} 
\multicolumn{1}{|c|}{}                      & LPIPS$\downarrow$ & 0.746 & 0.325 & 0.238 & 0.142 & 0.893 & 0.360 & 0.334 & 0.182 & 0.146 & 0.274 & 0.314 & 0.235 & 0.089 & 0.085 & 0.085 & 0.062 & 0.097 & 0.084 & 0.052 \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{SHIQ}} & PSNR$\uparrow$  & 5.47  & 19.34 & 24.77 & 27.30 & 5.31  & 12.24 & 21.78 & 23.80 & 16.40 & 25.49 & 22.05 & 14.74 & 37.97 & 30.92 & 26.80 & 31.57 & 34.57 & 21.42 & 33.60 \\ \cline{2-21} 
\multicolumn{1}{|c|}{}                      & SSIM$\uparrow$  & 0.483 & 0.679 & 0.890 & 0.917 & 0.556 & 0.491 & 0.700 & 0.909 & 0.724 & 0.858 & 0.832 & 0.724 & 0.980 & 0.963 & 0.935 & 0.965 & 0.972 & 0.903 & 0.974 \\ \cline{2-21} 
\multicolumn{1}{|c|}{}                      & LPIPS$\downarrow$ & 0.823 & 0.471 & 0.200 & 0.102 & 0.837 & 0.473 & 0.460 & 0.154 & 0.306 & 0.201 & 0.287 & 0.283 & 0.034 & 0.058 & 0.091 & 0.059 & 0.044 & 0.165 & 0.041 \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{SSHR}} & PSNR$\uparrow$  & 10.87 & 28.47 & 24.53 & 24.00 & 10.72 & 27.13 & 29.46 & 18.62 & 26.15 & 26.95 & 23.38 & 26.16 & 26.43 & 31.07 & 28.40 & 33.45 & 33.32 & 31.57 & 36.29 \\ \cline{2-21} 
\multicolumn{1}{|c|}{}                      & SSIM$\uparrow$  & 0.778 & 0.916 & 0.896 & 0.891 & 0.781 & 0.914 & 0.924 & 0.804 & 0.910 & 0.902 & 0.886 & 0.916 & 0.301 & 0.941 & 0.874 & 0.951 & 0.950 & 0.944 & 0.964 \\ \cline{2-21} 
\multicolumn{1}{|c|}{}                      & LPIPS$\downarrow$ & 0.357 & 0.094 & 0.101 & 0.094 & 0.358 & 0.077 & 0.076 & 0.281 & 0.076 & 0.094 & 0.110 & 0.060 & 0.059 & 0.041 & 0.092 & 0.028 & 0.036 & 0.035 & 0.023 \\ \hline
\end{tabular}
}
\label{tab:quan_horiztl}
\end{table*}
